Leveraging Multiple Transmissions and Receptions for Channel-Agnostic Deep Learning-Based Network Device Classification

The accurate identification of wireless devices is critical for enabling automated network access monitoring and authenticated data communication in large-scale networks; e.g., IoT. RF fingerprinting has emerged as a solution for device identification by leveraging the transmitter unique manufacturing impairments. Although deep learning is proven efficient in classifying devices based on the hardware impairments fingerprints, DL models perform poorly due to channel variations. That is, although training and testing neural networks using data generated during the same period achieve reliable classification, testing them on data generated at different times degrades the accuracy substantially, an already well recognized problem within the community. To the best of our knowledge, we are the first to propose to leverage MIMO capabilities to mitigate the channel effect and provide a channel-resilient device classification. We show that for AWGN channels, combining multiple received signals improves the testing accuracy by up to $30\%$. We also show that for Rayleigh channels, blind channel estimation enabled by MIMO increases the testing accuracy by up to $40\%$ when the models are trained and tested over the same channel, and by up to $60\%$ when the models are tested on a channel that is different from that used for training.

==> Fading-thesis.tex <==
\end{equation}
Equation~\eqref{eq7} sets the first requirement for channel uniqueness by assuming that $(\mathbf{\Tilde{C}})$ is full raw rank, and therefore $(\mathbf{\Tilde{C}\Tilde{C}}^H)$ is non-singular. Such assumption is valid for any well designed STBC, as raw rank-deficient codes imply the existence of redundant transmitting antennas and hence wasted diversity.\\
From Equation~\eqref{eq6}, and Equation~\eqref{eq7}, we get:
\begin{equation} \label{eq8}
    (\mathbf{I}_{2nK} \otimes \mathbf{H})\mathbf{\Gamma} \mathbf{q}=0
\end{equation}
where
\[\mathbf{\Gamma} \triangleq 
\begin{bmatrix}
(\mathbf{I}_{2n}\otimes \mathbf{C}_1 - \sum_{i=1}^{K} (\mathbf{C}_i^H(\mathbf{\Tilde{C}\Tilde{C}}^H)^{-1} \mathbf{C}_1)^T \otimes \mathbf{C}_i\\
(\mathbf{I}_{2n}\otimes \mathbf{C}_2 - \sum_{i=1}^{K} (\mathbf{C}_i^H(\mathbf{\Tilde{C}\Tilde{C}}^H)^{-1} \mathbf{C}_2)^T \otimes \mathbf{C}_i\\
\vdots \\
(\mathbf{I}_{2n}\otimes \mathbf{C}_k - \sum_{i=1}^{K} (\mathbf{C}_i^H(\mathbf{\Tilde{C}\Tilde{C}}^H)^{-1} \mathbf{C}_k)^T \otimes \mathbf{C}_i \\
\end{bmatrix}
\]

\begin{equation} \label{eq9}
\begin{split}
        \mathbf{\hat h}= (\mathbf{I}_M \otimes \mathbf{H}) \mathbf{\Phi} \mathbf{q}
    \end{split}
\end{equation}
where 
\[\mathbf{\Phi} \triangleq \sum_{i=1}^K (\mathbf{C}_i^H(\mathbf{\Tilde{C}\Tilde{C}}^H)^{-1} \mathbf{C}_1)^T \otimes \mathbf{C}_i\]
%
Equation~\eqref{eq8}, and Equation~\eqref{eq9} derived in~\cite{ammar_blind_2007} represent all the possible solutions for the channel matrix $\mathbf{H}$.
If $\mathbf{\Omega}$ is the space formed by the solution set for $\mathbf{\hat{h}}$ in Equation~\eqref{eq8} and Equation~\eqref{eq9}, then the channel is uniquely identifiable up to a complex scalar if and only if $dim(\mathbf{\Omega})=1$~\cite{ammar_blind_2007}. For instance, if $dim(\mathbf{\Omega})=2$, then the solution is not unique, and it is not possible to blindly determine which of the two possible solutions is the actual channel. 
Therefore, finding $dim(\mathbf{\Omega})$ in terms of the STBC and without involving the unknown channel matrix is essential for verifying whether the channel is identifiable or not. In addition, determining $dim(\mathbf{\Omega})$ identifies the minimum hardware requirements that allow blind channel estimation with minimum amount of uncertainty.
%
$dim(\mathbf{\Omega})$ is derived in~\cite{ammar_blind_2007} from Equation~\eqref{eq8}, and Equation~\eqref{eq9} for any channel $\mathbf{H}$:
\begin{equation} \label{eq10}
\begin{split}
        &dim(\mathbf{\Omega})= rank(\begin{bmatrix}
\mathbf{\Gamma}^H  & \mathbf{\Phi}^H
\end{bmatrix}^H)-rank(\mathbf{\Gamma})\\
&-dim(Null(\mathbf{I}_{2nK+M}\otimes \mathbf{H}) \cap Range(\begin{bmatrix}
\mathbf{\Gamma}^H  & \mathbf{\Phi}^H
\end{bmatrix}^H))\\
&+dim(Null(\mathbf{I}_{2nK}\otimes \mathbf{H} \cap Range(\mathbf{\Gamma})))
\end{split}
\end{equation}
By defining the variables $\rho$ and $\mathcal{R}$ such that:
\begin{equation*}
\begin{split}
\rho & \triangleq rank(\begin{bmatrix}
\mathbf{\Gamma}^H  & \mathbf{\Phi}^H
\end{bmatrix}^H)-rank(\mathbf{\Gamma}),\\
\mathcal{R} & \triangleq dim(Null(\mathbf{I}_{2nK} \otimes \mathbf{H}) \cap Range(\mathbf{\Gamma}))\\
&-dim(Null(\mathbf{I}_{2nK+M}\otimes \mathbf{H}) \cap Range(\begin{bmatrix}
\mathbf{\Gamma}^H  & \mathbf{\Phi}^H
\end{bmatrix}^H))\\
\end{split}
\end{equation*}
Equation~\eqref{eq10} is written as:
\begin{equation} \label{eq11}
dim(\mathbf{\Omega})= \rho + \mathcal{R}
\end{equation}
Equation~\eqref{eq11} is considered the identifiability condition of the channel in~\cite{ammar_blind_2007}, and it indicates the two sources of the channel uncertainties. One source is the STBC, quantified by $\rho$, and it could be addressed by using an STBC where $\rho = 1$ which will control the number of transmitting antennas. The second source of ambiguity is quantified by the residual term $\mathcal{R}$. However, this term depends on the unknown channel matrix $\mathbf{H}$. Once the channel matrix is decoupled from the identifiability condition, $\rho$ could be set to one by choosing an appropriate STBC; hence the channel is identifiable up to a complex scalar ambiguity.
The two approaches to decouple the channel matrix are either to assume a full rank channel matrix, or to find the conditions on the channel rank that set the residual term to zero.
\paragraph{Full Column Rank Channels}
Assuming the $\mathbf{H}$ is a full column rank channel, i.e. $rank(\mathbf{H}) = M$, the trivial right null space of $\mathbf{H}$ reduces Equation~\eqref{eq11} to: 
\begin{equation}\label{eq12}
    dim(\mathbf{\Omega})= \rho
\end{equation}
hence, the channel identifiability depends only on the STBC i.e. $\rho$.
\paragraph{Column Rank-Deficient Channels}
In Equation~\eqref{eq12}, if
\begin{equation} \label{eq13}
Null(\mathbf{I}_{2nK} \otimes \mathbf{H} \cap Range(\mathbf{\Gamma})) = \{0\}
\end{equation}
and
\begin{equation}\label{eq14}
Null(\mathbf{I}_{2nK+M}\otimes \mathbf{H}) \cap Range(\begin{bmatrix}
\mathbf{\Gamma}^H  & \mathbf{\Phi}^H
\end{bmatrix}^H) = \{0\}
\end{equation}
then the channel identifiability depends only on the STBC.\\ 
To find the conditions under which Equation~\eqref{eq13} holds true, a vector $\mathbf{z}\in Null(\mathbf{I}_{2nK} \otimes \mathbf{H} \cap Range(\mathbf{\Gamma})) $ is assumed, i.e.:
\begin{equation} \label{eq15}
\begin{split}
    (\mathbf{I}_{2nK}\otimes \mathbf{H})\mathbf{z}=0\\
    \exists \mathbf{u} \notin Null(\mathbf{\Gamma})\ s.t.\ \mathbf{\Gamma} \mathbf{u}=\mathbf{z}
    \end{split}
\end{equation}
to relate $\mathbf{z}$ with the STBC represented by $\mathbf{\Gamma}$, Equation~\eqref{eq15} is reordered as follows:
\begin{equation}\label{eq16}
\begin{split}
\mathbf{H}\mathbf{Z}&= \mathbf{0} \\
\mathbf{Z}= \mathbf{\Tilde \Gamma}\mathbf{(I}_{2nK} \otimes \mathbf{u}), & \quad \mathbf{u} \notin Null(\mathbf{\Gamma})
\end{split}
\end{equation}
where 
\[\mathbf{\Tilde \Gamma} = \begin{bmatrix}
\mathbf{\Gamma}_1 & \mathbf{\Gamma}_2 & \hdots & \mathbf{\Gamma}_{2nK}
\end{bmatrix}\]
and $\mathbf{Z}$ is an $M\times2nK$ matrix such that $vec(\mathbf{Z})=\mathbf{z}$.\\
To ensure that $\mathbf{z}$ lies in the column space of $\mathbf{\Gamma}$, $\mathbf{Z}$ must have a minimum rank $r_{min}$~\cite{ammar_blind_2007}:
\begin{equation} \label{eq17}
r_{min} \triangleq \min_{\mathbf{u}\notin Null(\mathbf{\Gamma})} \quad rank(\mathbf{\Tilde \Gamma}(\mathbf{I}_{2nK} \otimes \mathbf{u})).
\end{equation}
In addition, $rank(\mathbf{Z})$ cannot exceed the dimension on the null space of $\mathbf{H}$. Hence we get:
\begin{equation}\label{eq18}
r_{min}\leq rank(\mathbf{Z}) \leq dim(Null(\mathbf{H})) = M-rank(\mathbf{H})
\end{equation}
therefore,
\begin{equation} \label{eq19}
\begin{split}
& if \quad rank(\mathbf{H})> M-r_{min},\\
& then \quad Null(\mathbf{I}_{2nK} \otimes \mathbf{H} \cap Range(\mathbf{\Gamma})) = \{0\}.
\end{split}
\end{equation}
Similarly, for Equation~\eqref{eq14} we get an analogy to~\eqref{eq19}:
\begin{equation} \label{eq20}
\begin{split}
& if \quad rank(\mathbf{H})> M-r_{min}^\prime \\
& then \quad Null(\mathbf{I}_{2nK+M}\otimes\mathbf{H})
\cap  Range(\begin{bmatrix}
\mathbf{\Gamma}^H  & \mathbf{\Phi}^H
\end{bmatrix}^H)\\
&= \{0\}
\end{split}
\end{equation}
where 
\begin{equation}\label{eq21}
r_{min}^ \prime \triangleq \min_{\mathbf{u}\notin Null(\begin{bmatrix}
\mathbf{\Gamma}\\
\mathbf{\Phi}
\end{bmatrix})} \quad rank(\begin{bmatrix}
\mathbf{\Tilde \Gamma} & \mathbf{\Tilde \Phi}
\end{bmatrix} (\mathbf{I}_{2nK+M}\otimes \mathbf{u})).
\end{equation}
From Equation~\eqref{eq19} and Equation~\eqref{eq20} and with the identifiability condition in Equation~\eqref{eq11} we get that:
\begin{equation} \label{eq22}
\begin{split}
&if \quad rank(\mathbf{H})> M- min(r_{min}^\prime, r_{min}) \\
&then \quad dim(\mathbf{\Omega})= \rho.
\end{split}
\end{equation}
It is clear that $r_{min}$, $r_{min}^\prime$ depends on the STBC alone. Table~\ref{Tb1} shows The values of $r_{min}$, $r_{min}^\prime$ for some generic STBCs obtained from solving the optimization problems in Equation~\eqref{eq17} and Equation~\eqref{eq21}~\cite{ammar_blind_2007}.
Given that $rank(\mathbf{H})= min(M,L)$, these conditions on the channel rank constrain the minimum number of receiving antennas required to estimate the transmitted signal blindly such that:
\[L \geq M-r_{min}+1.\]
For instance, using Tarokh STBC $\mathcal{O}_3$ in Table~\ref{Tb1} to transmit QPSK symbols requires at least 3 receiving antennas for the channel to be blindly estimated up to a complex scalar ambiguity.
\begin{table}\scriptsize
\centering % centering table
\caption{\small Summary of $r_\text{min}$ for Different STBCs \cite{ammar_blind_2007}} %title of the table
\begin{tabular}{|c|c|c|c|c|c|} % creating five columns
\hline %inserting double-line
STBC & $(M,n,K)$ & $dim(\mathbf{\omega})$ & $r_\text{min}$ & $r_\text{min}^\prime$ & rank(C)\\
\hline % inserts single-line
$\mathcal{O}_1$ (Alamouti) & $(2,2,2)$ & 4 & 1 & 2 & 4\\ 
\hline
$\mathcal{O}_2$ (Tarokh) & $(3,3,4)$ & 1 & 3 & 3 & 6\\
\hline
$\mathcal{O}_3$ (Tarokh) & $(3,4,8)$ & 1 & 1 & 3 & 8\\ % [1ex] adds vertical space
\hline % inserts single-line
\end{tabular}
\label{Tb1}
\end{table}
\subsubsection{The Blind Estimation Algorithm}
Considering a MIMO transmission link equipped with the minimum hardware requirements that allow the channel to be blindly estimated from the received signal up to a complex scalar ambiguity as in~\cite{ammar_blind_2007}. When the link is sending an STBC signal and the received signal has a non-trivial left null space, we obtain the blind equation~\eqref{eq4}~\cite{ammar_blind_2007}. The blind algorithm proposed in~\cite{ammar_blind_2007} starts By reshaping Equation~\eqref{eq4} using the vector property of the Kronecker product we get:
\begin{equation} \label{eq23}
    \mathbf{C}^T \otimes \mathbf{N}^H_L  \cdot vec(\mathbf{I}_K\otimes \mathbf{H})=0
\end{equation}
where $\{.\}^T$ denotes the transpose operation.
To decouple the vector form of the unknown $\mathbf{H}$, we rewrite Equation~\eqref{eq23} as:
\begin{multline} \label{eq24}
vec(\mathbf{I}_K \otimes \mathbf{H})  =\begin{bmatrix}
                    \mathbf{I}_M \otimes \mathbf{E}_1 \\
                    \mathbf{I}_M \otimes \mathbf{E}_2 \\
                    \vdots \\
                    \mathbf{I}_M \otimes \mathbf{E}_3 \\
                    \end{bmatrix} \mathbf{h}\\
\mathbf{E}_k  \triangleq \begin{bmatrix}
                      \mathbf{0}_{L(k-1)\times L} \\
                           \hline\\
                            \mathbf{I}_L \\
                            \hline \\
                          \mathbf{0}_{L(K-k)\times L} 
                           \end{bmatrix}, \quad K =1,\hdots,K
\end{multline}
then we substitute Equation~\eqref{eq24} in Eqaution~\eqref{eq23} to get:
\begin{equation} \label{eq25}
   \overbrace{(\sum_{k=1}^{K} \mathbf{C}^T_k \otimes (\mathbf{N}^H_L \mathbf{E}_k))}^ {\triangleq \mathbf{\Delta}} \mathbf{h}= 0.
\end{equation}
Equation~\eqref{eq25} shows that $\mathbf{h}$ lies in the right null space of $\mathbf{\Delta}$, and since the channel is identifiable up to a single complex scalar ambiguity, $\mathbf{h}$ spans the null space of $\mathbf{\Delta}$.
Singular value decomposition can be used to find the basis of the null space of $\mathbf{\Delta}$, specifically, the right singular vector corresponding the the smallest singular value of $\mathbf{\Delta}$ is the estimated channel vector $\mathbf{\hat h}$ where:
\[\mathbf{\hat h}= \alpha \mathbf{h}, \quad \alpha \in \mathbb{C} \]
%
Practically, the received signal matrix $\mathbf{R}$ is affected by additive white Gaussian noise, so it is required to separate the noise and the signal subspaces before using the blind algorithm~\cite{ammar_blind_2002} using the subspace approach~\cite{moulines_subspace_1995}.
To solve the remaining ambiguity and completely estimate the channel, additional information about the channel matrix is obtained by sending pilots known for the receiver. The pilots assist the blind algorithm to completely identify the channel~\cite{ammar_blind_2007}. 









==> Performance_evaluation.tex <==
Here is how to add a table:
\begin{table}\scriptsize
\centering % centering table
\caption{\small PAYPHONES IN THE FIVE BOROUGHS OF NYC \cite{sinky2017responsive}} %title of the table
\begin{tabular}{c rrrr} % creating eight columns
\hline %inserting double-line
Borough & \# Payphones & Avg. distance & BSs\\
\hline % inserts single-line
Manhattan & 3409 & 42.3m & 50\\ % Entering row contents
Queens & 1042 & 136.8m & 25\\
Brooklyn & 1004 & 150.8m & 25\\ % [1ex] adds vertical space
Bronx & 591 & 125.5m & 20\\
Staten Island & 51  &606m & 10\\
Total & 6097 & 212.5m & 130\\
\hline % inserts single-line
\end{tabular}
\label{tab:hresult}
\end{table}
%\vspace{-0.15in}

%Here is how to add a figure:

Fig.~\ref{fig:dist} shows ...
\begin{figure}[h]
\centerline{
    \subfigure[Intrinsic objective]
   {\includegraphics[width=1\columnwidth]{UserDistribution_gj.eps}
    \label{subfig:dist-gj}}}
    %
\centerline{
    \subfigure[Global objective]
    {\includegraphics[width=1\columnwidth]{UserDistribution_G.eps}
    \label{subfig:dist-G}}}
    %
\centerline{
    \subfigure[Proposed objective ]
    {\includegraphics[width=1\columnwidth]{UserDistribution_Dj.eps}
    \label{subfig:dist-D}}}
%
\caption{Distribution of the $500$ agents across the $m=10$ different bands.} 
\label{fig:dist}
\end{figure}
%

==> Proposed_technique.tex <==
We propose to leverage the MIMO capabilities to enable channel-agnostic RF data driven fingerprinting using Convolution Neural Network (CNN) based deep learning. Our proposed techniques address RF signal distortions caused by AWGN and flat fading channels using the aforementioned methods explained in Section~\ref{subsec:AWGN}, Section~\ref{subsec:Fading}, respectively.

\subsubsection{Mitigating AWGN Channel}
For AWGN channels we use the SIMO system where the receiver is equipped with multiple antennas, and we propose averaging the multiple received signals as explained in Section~\ref{subsec:AWGN} in order to achieve an SNR gain that mitigates the channel noise and compensate the reduced SNR. Intuitively, the training phase of the CNN on the sampled averaged signal is expected to be more oblivious to the noise effect which appears as an increase in the training accuracy. In addition, testing the CNN in an AWGN channel with a lower SNR using the averaged signal is less affected by the noise, and the reduction in the testing accuracy due to the change of the channel is less compared to the SISO system. 
\subsubsection{Mitigating Flat Fading Channel}
For flat fading channels, we propose leveraging the blind partial estimation enabled by the MIMO system proposed in~\cite{ammar_blind_2007} and explained in Section~\ref{subsec:Fading}. 
To enable blind channel estimation and reliable RF classification, we suggest to set the MIMO hardware and the STBC at the minimum requirements to guarantee a blind channel estimation from the received signals up to a single complex ambiguity, i.e. $\rho=1$. Once the channel is blindly estimated up to a single complex ambiguity, the resolved signals are sampled and used for training and testing the CNN model used for classification. In our proposed technique we use CNN for classification, and we leverage the CNN ability to learn from training data and generalize on unseen data to overcome the remaining ambiguity and capture the impairments effect on the reconstructed waveforms.




==> old-MIMO_Background-old.tex <==
Multiple-Input Multiple-Output (MIMO) systems have emerged as a most promising technology to achieve higher data rates, better quality of service, and higher network capacity by using multiple antennas at the transmitting end as well as at the receiving end \cite{foschini_layered_1996, winters_diversity_1998}. 
%The core concept of MIMO is that combining signals sampled in the spatial domain at both ends would either create effective multiple parallel spatial data streams, therefore increasing the data rate, or add spatial diversity to improve the quality of the communication \cite{clerckx_mimo_2013}.
The concept of spatial diversity is that the SNR is significantly improved by combining the outputs of decorrelated antenna elements in presence of fading caused by multipath propagation \cite{clerckx_mimo_2013}. %Each version of the received signal is called a diversity branch, and if the branches are affected by independent fading, the probability that all branches will have a deteriorated SNR at the same time will decrease drastically \cite{}. 
The increase in average output SNR relative to the single-branch average SNR is defined as Diversity Gain \cite{clerckx_mimo_2013}. 
\subsubsection{Receive Diversity}
The concept of Receive Diversity was introduced via SIMO systems, where a single antenna is used at the transmitting end while multiple antennas are used at the receiving end. Receive diversity gain is obtained by different combining methods:
\begin{itemize}
  \item Selection combining: the combiner selects the branch with the highest SNR which is then used for detection.
  \item Gain combining: the signal used for detection is an optimal linear combination of all branches to increase the overall SNR\cite{clerckx_mimo_2013}.
\end{itemize}
The overall increase in the SNR at the output of the SIMO system thanks to any of the combining schemes appears as improvement in the Symbol Error Probability in case of considering Symbol Error Probability as the performance metric.\cite{win_virtual_2001}. In RF fingerprinting systems where the fingerprinting accuracy is a main performance metric, the SNR diversity gain may appear as an increase in the fingerprinting accuracy and the receive diversity may mitigate the degradation of the system accuracy that happens when the system is trained or implemented in AWGN channels with low SNR. Therefore, MIMO system stands out as a strong candidate solution that is worthy of deep investigation when it comes to mitigating the channel effect for a channel-resilient RF fingerprinting.

\subsubsection{Transmit Diversity and Space-Time Block Coding}
Space-Time Block Codes (STBC) have been established as an efficient method to enhance wireless communication systems performance. STBCs are applied by spreading information symbols in space and time using multiple transmitting antennas \cite{tarokh_space-time_1999, foschini_layered_1996,  winters_diversity_1998, clerckx_mimo_2013}.
Thanks to the STBCs properties to ensure transmit diversity, the Blind estimation of the channel by observing only the received signals is possible \cite{swindlehurst_blind_2002, ammar_blind_2007, peken_blind_2017}. Leveraging this blind estimation capability of a MIMO system with STBC, we can build a channel-resilient RF fingerprinting CNN model.



